An Economic Analysis of User-Privacy Options in Ad-Supported Services

We analyze the value to e-commerce website operators of offering privacy options to users, e.g., of allowing users to opt out of ad targeting. In particular, we assume that site operators have some control over the cost that a privacy option imposes on users and ask when it is to their advantage to make such costs low. We consider both the case of a single site and the case of multiple sites that compete both for users who value privacy highly and for users who value it less. One of our main results in the case of a single site is that, under normally distributed utilities, if a privacy-sensitive user is worth at least $\sqrt{2} - 1$ times as much to advertisers as a privacy-insensitive user, the site operator should strive to make the cost of a privacy option as low as possible. In the case of multiple sites, we show how a Prisoner's-Dilemma situation can arise: In the equilibrium in which both sites are obliged to offer a privacy option at minimal cost, both sites obtain lower revenue than they would if they colluded and neither offered a privacy option.

==> conclusion.tex <==
\section{Conclusion}
The results of Sections~\ref{sec:single} and \ref{sec:2player} suggest that 
website operators could have their cake and eat it, too. By carefully 
controlling the cost to users of opting out of targeted ads, they could 
maximize their revenue and respect their users' privacy concerns. Putting this 
approach into practice would require surmounting at least two major obstacles.

First, a service provider would need a good estimate of the parameter $\gamma$, 
{\it i.e.}, the fraction of the revenue derived from a targeted user that can 
be derived from a private user. The value of $\gamma$ is closely related to the 
extent to which click-through and conversion rates are improved by various 
forms of ad targeting, which in turn is still the subject of intensive, ongoing 
research.

Second, the service provider would need to translate the abstract ``cost'' 
$c_i$ of our economic analysis into a concrete privacy-enforcement tool that 
can be installed and used at a cost of $c_i$. It may suffice to be able to 
choose between two technological options, one of which is clearly more costly 
to users than the other, but even this would be nontrivial given the state of 
the art of privacy enforcement.


==> related.tex <==
\section{Related Work}\label{sec:related}

To the best of our knowledge, we are the first to study the question of when it is to 
advantage of website operators to minimize the cost of providing users with privacy options.  
However, several related aspects of web users' ability to control their personal information 
have been studied.

Riederer {\it et al.}~\cite{RECKR11} propose a market for personal information based on the 
notion of {\it transactional privacy}.  Users decide what information about themselves should 
be for sale, and aggregators buy access to users' information and use it to decide what ads 
to serve to each user.  The information market that connects users and aggregators, handles 
payments, and protects privacy achieves truthfulness and efficiency using an unlimited-supply 
auction.

Carrascal {\it et al.}~\cite{CRECO12} use {\it experience sampling} to study the monetary value 
that users place on difference types of personal information.  They find, for example, that 
users place a significantly higher value on information about their offline behavior than they 
do on information about their browsing behavior.  Among categories of online information, they 
value financial and social-network information more highly than search and shopping information.

Iyer, Soberman, and Villas-Boas~\cite{ISVB05} consider advertising strategies in segmented markets, 
where competing firms can target ads to different segments.  They find that firms can increase 
profits by targeting more ads at consumers who have a strong preference for their product than 
at comparison shoppers who might be attracted to the competition.  Interestingly, targeted 
advertising produces higher profits regardless of whether the firms can price discriminate.  
Moreover, the ability to target advertising can be more valuable to firms in a competitive 
environment than the ability to price discriminate.

Telang, Rajan, and Mukhopadhyay~\cite{MRT04-Structure} address the question of why multiple 
providers of free, online search services can coexist for a long time.  In standard models 
of vertical (or quality) differentiation, a lower-quality product or service must sell for a 
lower price than its higher-quality competitor if it is to remain in the marketplace; if the prices 
are equal, all consumers choose the higher-quality alternative.  Similarly, in standard models 
of horizontal (or taste) differentiation, sustained differentiation among products or services occurs
when users incur high transportation costs.  Yet, neither price nor transportation cost is a strategic
variable in online search.  Telang, Rajan, and Mukhopadhyay point out that, although the quality of
one search service may clearly be higher than that of its competitors {\it on average}, the quality of
results of {\it a particular search by a particular user} is highly variable and inherently stochastic.
Thus, there is a nontrivial probability that a user will be dissatisfied with the results of a 
particular search and wish to search again for the same information, using a different search service.
It is precisely the zero-price, zero-transportation-cost nature of the user's task that may cause him
to use more than one search service in a single session.  In the aggregate, this feature creates
residual demand for lower-quality search services, allowing them to coexist with their higher-quality
competitor.



